Solving Seismic Wave Equations on Variable Velocity Models with Fourier Neural Operator

In the study of subsurface seismic imaging, solving the acoustic wave equation is a pivotal component in existing models. The advancement of deep learning enables solving partial differential equations, including wave equations, by applying neural networks to identify the mapping between the inputs and the solution. This approach can be faster than traditional numerical methods when numerous instances are to be solved. Previous works that concentrate on solving the wave equation by neural networks consider either a single velocity model or multiple simple velocity models, which is restricted in practice. Instead, inspired by the idea of operator learning, this work leverages the Fourier neural operator (FNO) to effectively learn the frequency domain seismic wavefields under the context of variable velocity models. We also propose a new framework paralleled Fourier neural operator (PFNO) for efficiently training the FNO-based solver given multiple source locations and frequencies. Numerical experiments demonstrate the high accuracy of both FNO and PFNO with complicated velocity models in the OpenFWI datasets. Furthermore, the cross-dataset generalization test verifies that PFNO adapts to out-of-distribution velocity models. Moreover, PFNO has robust performance in the presence of random noise in the labels. Finally, PFNO admits higher computational efficiency on large-scale testing datasets than the traditional finite-difference method. The aforementioned advantages endow the FNO-based solver with the potential to build powerful models for research on seismic waves.

==> discussion.tex <==
\section{Discussion}
The propagation of seismic waves implies geological subsurface information. Therefore, understanding wave propagation, which is governed by the wave equation, on velocity models with certain features has far-reaching benefits in the study of seismology. In practice, one might encounter thousands or even tens of thousands of velocity models. However, it can be computationally expensive for traditional solvers to solve the wave equation with such a large number of velocity models. In pursuit of accurate and fast numerical solvers based on deep learning, we introduce FNO and PFNO that efficiently solve the Helmholtz equation on multiple velocity models. 

%This work focuses on the forward problem and demonstrates the efficiency of FNO-based solvers using datasets from the OpenFWI dataset collection. More specifically, the $6$ datasets, which belong to $3$ families, compose of velocity models with different features, including faults and flat or curved layers. The first experiment shows the high accuracy of PFNO under the multi-source-location and multi-frequency setting. Compared with single FNO and ForwardNet, it better captures the complicated scatters in the wavefields. We then examine the generalization of PFNO with velocity models in different datasets. This verifies its practicality since one does not need to retrain the model provided that the unseen velocity models do not differ immoderately from the ones used in training. Another pragmatic property of the FNO-based solvers is that they are insensitive to the measurement errors of the receiver. By injecting random noise into the ground truth wavefields, we simulate the measurement errors. PFNO, nevertheless, performs consistently under random noise. Notably, FNO and PFNO have a significant edge of speed over the ``optimal" 9-point method, given a large number of velocity models. In practice, this enables them to serve as a building block of other models in the related research.  

Accuracy is a key factor when evaluating a numerical solver for differential equations. In this work, our numerical experiments show that FNO-based solvers achieve high accuracy on variable velocity models. The accuracy stems from the expressive power of the neural operator defined as a composition of integrals~\cite{li2020fourier,li2020neural}, in each of which a neural network parameterizes a generalized Green's function of a (differential) operator. The activation functions provide nonlinearity to the composition, bolstering its ability to approximate complicated functional mappings in infinite-dimensional space. In our context, velocity is not a fixed parameter but a function of location $(x, ~z)$. Hence, we leverage the neural operator to map the velocity to the solution of the Helmholtz equation, which is also a function of location. With $4$ Fourier layers~\cite{li2020fourier}, FNO is capable of approximating the complicated mapping between the input velocity models and the frequency domain wavefield. On the $6$ datasets in OpenFWI, FNO yields accurate predicted wavefields, even for high frequency data as illustrated in~\Cref{fig:wavefield_freqs}. Multiple source locations and frequencies need to be considered in practice. The performance of FNO is unsatisfactory if we naively add the source location and the frequency into the input due to the increasing complexity of the mapping. Consequently, much more wavefield data based on different source locations and frequencies must be incorporated for the training. However, the storage required is infeasible, given such a large number of velocity models.  As a countermeasure, PFNO lets data of different frequencies be treated by specialized FNO. In this architecture, the frequency is no longer a variable parameter in the input. Then, PFNO is trained under the multi-source-location and multi-frequency setting, and it outperforms FNO and ForwardNet on all the testing datasets. In particular, ForwardNet considers the velocity models and the wavefields as pure images. Therefore, it does not exploit any information from the Helmholtz equation. In addition, it is mesh-dependent since it does not take the location as a part of the input. Despite still being a purely data-driven method, PFNO implicitly uses the equation by generalizing the idea of Green's function. Following this discussion, we state that the maximum misfit might be large in the exceedingly irregular parts of the wavefield, although the error is small in the average sense. A potential improvement is to explicitly embed the Helmholtz equation in the training, as in PINN~\cite{raissi2019physics}. 

The generalization of FNO-based solvers affects their wide applicabilities, since poor generalization amounts to retraining the model when a new dataset is to be solved. We expect PFNO to adapt to unseen velocity models and still be able to make accurate predictions. The cross-dataset generalization test is performed for verification, where testing samples come from other datasets. The result is consistent with our expectation as PFNO generalizes well to the velocity models that share features in common with the ones in the training set. In contrast, generalization should not be expected if the velocity models differ significantly. For example, the PFNO trained on \emph{CurveFault-B} generalizes to \emph{Style-B} because the velocity models have curved structures in both. However, it has a poor performance on \emph{FlatVel-B} since the velocity models have flat layers, and the velocity values are distributed randomly across layers. Moreover, we also investigated FNO's generalization on frequency while maintaining its generalization on velocity. The experiments use $30$ frequencies for training and $5$ frequencies for testing. FNO only has weak generalization in high frequency wavefields. This is because wavefields of high frequencies look alike, while low frequency wavefields are disparate from one another. The lack of generalization on frequency results from insufficient diversity of frequency. Improving it requires us to incorporate data of more frequencies with a smaller interval. In our experiments, $30$ frequencies are incorporated with a $1$Hz interval. We might need to reduce the interval to $0.1$Hz. Certainly, the size of the dataset will grow considerably when more frequencies are incorporated, which restricts the number of velocity models given a fixed storage space. Hence, it remains an open research topic to improve the generalization on frequency with a limited increase in the dataset size.  

Another pragmatic property of the FNO-based solvers is that they are insensitive to the measurement error of the receiver since the error is almost inevitable in practice. By injecting random noise into the ground truth wavefields, we simulate the measurement error. The magnitude of the error is controlled by the standard deviation of the random noise. Although the training error slightly rises, the testing error of PFNO remains stable. A possible explanation is that the random noise prevents PFNO from overfitting the training data and enables it to better generalize to the testing data. In other words, PFNO is robust against random noise. 

Finally, we address the computational efficiency of FNO and PFNO. The numerical tests demonstrate that they have a significant edge of speed over the ``optimal" 9-point method, given a large number of velocity models. More specifically, FNO prevails over the ``optimal" 9-point method when we need to solve thousands of velocity models. Under the multi-source-location and multi-frequency setting, PFNO gains the edge even though only hundreds of velocity models are present. The speed-up is the result of comprehensive factors. First of all, FNO and PFNO leverage FFT with complexity $O(n \log(n))$ for fast computation and truncate the number of Fourier modes used. In terms of the hardware, paralleling computing is efficiently utilized when we harness multiple GPUs. Although it takes a couple of hours for training, the inference (testing) process only takes seconds to handle thousands of velocity models. In practice, this speed-up enables them to serve as a building block for other models in the related research.

To further elaborate on the contribution to the community, we emphasize the potential of the FNO-based solvers in inverse problems. Full waveform inversion is one of the commonly used techniques to invert the subsurface structures in regional exploration surveys, carbon capture and storage sites, Earth interior imaging, and many other applications. A successful FWI requires hundreds of forward and adjoint wavefield simulation steps that are implemented in the velocity models of similar distributions. Our proposed FNO and PFNO solvers can instantly solve the forward wavefield in the frequency domain once trained. The adjoint wavefield, which requires the ability to deal with multiple source functions (adjoint sources), may need further development of the proposed PFNO network.
